On Efficient Variants of Segment Anything Model: A Survey

The Segment Anything Model (SAM) is a foundational model for image segmentation tasks, known for its strong generalization across diverse applications. However, its impressive performance comes with significant computational and resource demands, making it challenging to deploy in resource-limited environments such as edge devices. To address this, a variety of SAM variants have been proposed to enhance efficiency while keeping accuracy. This survey provides the first comprehensive review of these efficient SAM variants. We begin by exploring the motivations driving this research. We then present core techniques used in SAM and model acceleration. This is followed by a detailed exploration of SAM acceleration strategies, categorized by approach, and a discussion of several future research directions. Finally, we offer a unified and extensive evaluation of these methods across various hardware, assessing their efficiency and accuracy on representative benchmarks, and providing a clear comparison of their overall performance.

==> figs/response_seginw.tex <==
\begin{table*}[ht]
\centering
\small
\setlength{\tabcolsep}{3pt}
\caption*{Table 10: Quantitative results of zero-shot instance segmentation on SGinW benchmark with GroundingDINO as the object detector.We report variants' Average Precision (AP) on each dataset and mean AP over all 25 datasets.}
\label{tab:sginw_transposed_rotated}
\begin{tabular}{@{} l | *{16}{c} @{}}
\toprule
 {Dataset} & 
{\footnotesize \rotatebox{90}{ {SAM-H}}} & 
{\footnotesize \rotatebox{90}{ {SAMfast-H}}} & 
{\footnotesize \rotatebox{90}{ {sam2-B+}}} & 
{\footnotesize \rotatebox{90}{ {FastSAM}}} & 
{\footnotesize \rotatebox{90}{ {MobileSAM}}} & 
{\footnotesize \rotatebox{90}{ {EdgeSAM}}} & 
{\footnotesize \rotatebox{90}{ {EfficientSAM-Ti}}} & 
{\footnotesize \rotatebox{90}{ {EfficientSAM-S}}} & 
{\footnotesize \rotatebox{90}{ {RepViT-SAM}}} & 
{\footnotesize \rotatebox{90}{ {SlimSAM50}}} & 
{\footnotesize \rotatebox{90}{ {SlimSAM77}}} & 
{\footnotesize \rotatebox{90}{ {TinySAM}}} & 
{\footnotesize \rotatebox{90}{ {Q-TinySAM}}} & 
{\footnotesize \rotatebox{90}{ {EfficientViT-SAM-L0}}} & 
{\footnotesize \rotatebox{90}{ {EfficientViT-SAM-XL1}}} & 
{\footnotesize \rotatebox{90}{ {NanoSAM}}}  \\
\hline
 {Airplane-Parts}    & 35.3  & 35.2   & \textbf{36.6}   & 23.1      & 31.1       & 31.6      & 32.5            & 35.1           & 29.6      & 29.1       & 26.1       & 28.6     & 33.0       & 35.2               & 34.6               & 30.5      \\
 {Bottles}           & 65.7  & 65.2   & 66.5   & 59.6      & 64.1       & 64.9      & 63.4            & 64.8           & 65.1      & 63.8       & 64.0       & 64.6     & 63.1       & 66.5               & \textbf{67.1}               & 63.7      \\
 {Brain-Tumor}       & 11.7  & 11.7   & 11.2   & 2.1       & \textbf{12.2}       & 11.3      & 12.0            & 12.0           & 11.6      & 11.2       & 11.6       & 9.9      & 11.8       & 11.5               & 12.1               & 11.9      \\
 {Chicken}           & 85.9  & \textbf{86.8}   & 79.1   & 71.1      & 84.5       & 81.9      & 83.4            & 85.6           & 85.2      & 83.2       & 85.5       & 83.2     & 82.7       & 82.4               & 85.1               & 80.2      \\
 {Cows}              & 46.3  & 46.2   & \textbf{46.6}   & 17.0      & 42.7       & 40.1      & 43.3            & 45.3           & 42.2      & 43.0       & 41.5       & 38.2     & 41.4       & 43.5               & 45.3               & 40.5      \\
 {Electric-Shaver}   & 70.5  & 70.2   & \textbf{71.8}   & 49.4      & 66.3       & 65.2      & 66.2            & 68.5           & 64.2      & 58.1       & 63.9       & 59.9     & 65.6       & 69.8               & 70.6               & 64.2      \\
 {Elephants}         & 77.2  & \textbf{77.3}   & 76.2   & 61.3      & 70.5       & 68.4      & 70.7            & 74.1           & 70.0      & 68.6       & 70.1       & 64.3     & 68.4       & 72.2               & 74.8               & 68.1      \\
 {Fruits}            & 82.3  & \textbf{82.3}   & 80.7   & 81.5      & \textbf{82.3}       & 81.5      & 81.7            & 81.7           & 81.5      & 81.5       & 81.5       & 74.0     & 76.2       & 81.5               & 81.5               & \textbf{82.3}     \\
 {Garbage}           & 23.7  & 23.9   & \textbf{25.9}   & 10.1      & 22.7       & 20.5      & 19.7            & 23.3           & 21.9      & 17.8       & 19.2       & 16.9     & 21.8       & 23.5               & 23.2               & 20.7      \\
 {Ginger-Garlic}     & 45.8  & 45.8   & 44.9   & 28.3      & 43.6       & 40.2      & 44.6            & 45.7           & \textbf{47.0}      & 39.5       & 40.8       & 39.4     & 46.1       & 43.9               & 46.7               & 42.6      \\
 {Hand}              & 76.6  & 76.5   & 78.2   & \textbf{81.6}      & 73.2       & 71.0      & 69.3            & 76.7           & 73.0      & 71.9       & 74.6       & 66.9     & 70.8       & 74.1               & 75.3               & 70.7      \\
 {Hand-Metal}        & 81.4  & 81.1   & 78.8   & 70.6      & 80.9       & 78.5      & 76.4            & 80.0           & \textbf{81.3}      & 77.8       & 78.8       & 78.7     & 78.4       & 79.2               & 79.6               & 78.5      \\
 {HouseHold-Items}   & 60.1  & {60.1}   & {60.1}   & {60.1}      & 58.8       & 58.8      & 58.8            & {60.1}           & {60.1}      & {60.1}       & {60.1}       & 58.8     & 59.5       & {60.1}               & {60.1}               & 58.8      \\
 {House-Parts}       & 8.4   & \textbf{8.3}    & 8.0    & 6.6       & 8.1        & 8.1       & 8.0             & \textbf{8.3}            & \textbf{8.3}       & 8.1        & 8.0        & 7.8      & 7.9        & 8.2                & \textbf{8.3}                & 8.1       \\
 {Nutterfly-Squireel} & 70.0  & 69.4   & \textbf{80.8}   & 23.1      & 63.1       & 57.5      & 68.5            & 70.8           & 59.7      & 52.8       & 53.7       & 59.5     & 60.4       & 63.5               & 67.8               & 60.3      \\
 {Phones}            & 34.9  & 35.0   & 30.2   & 28.4      & 33.9       & 33.4      & 34.0            & \textbf{35.5}           & 34.5      & 33.8       & 35.3       & 34.2     & 34.5       & 34.3               & 34.8               & 31.4      \\
 {Poles}             & 23.3  & 23.3   & 15.6   & 5.1       & 16.6       & 15.9      & 20.0            & \textbf{27.7}           & 13.4      & 14.2       & 12.5       & 4.7      & 12.5       & 19.0               & 16.7               & 6.9       \\
 {Puppies}           & 50.1  & \textbf{50.1}   & \textbf{50.1}   & 28.4      & 45.0       & 44.6      & 46.7            & 47.8           & 45.0      & 46.0       & 46.8       & 38.6     & 44.2       & 45.8               & \textbf{50.1}               & 43.8      \\
 {Rail}              & 15.8  & 15.7   & 12.2   & 1.0       & 14.1       & 13.5      & 12.9            & 13.4           & 12.9      & 12.4       & 15.1       & \textbf{17.5}     & 15.4       & 17.5               & 16.7               & 13.1      \\
 {Salmon-Fillet}     & 36.2  & 36.3   & 19.7   & 24.5      & 29.9       & 31.7      & 12.4            & 21.8           & 25.2      & 27.8       & 28.0       & 18.3     & 27.0       & \textbf{39.2}               & 37.1               & 25.6      \\
 {Strawberry}        & 83.5  & 83.3   & 83.6   & 79.8      & 83.3       & 83.0      & 82.7            & 83.3           & 83.6      & 82.6       & 82.4       & \textbf{83.7}     & 82.6       & 83.4               & 83.6               & 83.5      \\
 {Tablets}           & 29.6  & \textbf{29.5}   & 27.1   & 29.0      & 28.7       & 28.4      & 29.0            & 29.3           & 28.9      & 28.7       & 28.7       & 28.6     & 28.5       & 28.8               & 28.8               & 28.7      \\
 {Toolkits}          & 20.9  & \textbf{20.9}   & 20.2   & 12.3      & 19.3       & 18.6      & 19.1            & 20.7           & 18.5      & 17.7       & 18.6       & 19.2     & 18.6       & 19.9               & 20.6               & 19.1      \\
 {Trash}             & 29.7  & \textbf{29.7}   & 27.7   & 27.3      & 28.8       & 28.3      & 28.8            & 29.1           & 28.9      & 28.6       & 28.7       & 27.5     & 28.2       & 28.7               & 29.3               & 28.6      \\
 {Watermelon}        & 64.9  & 64.5   & 63.7   & 44.4      & 63.5       & 66.2      & 64.6            & 66.1           & 62.7      & 62.1       & 63.7       & 62.8     & 63.4       & \textbf{67.3}               & 67.0               & 63.2      \\
\hline
 {Mean AP}           & 49.2  &  \textbf{49.1} & 47.8   & 37.0      & 46.7       & 45.7      & 45.9            & 48.3           & 46.2      & 44.8       & 45.6       & 43.4     & 45.7       & 48.0               & 48.7               & 45.0      \\
\bottomrule
\end{tabular}
\end{table*}

==> figs/response_summary.tex <==
\begin{table*}[ht]
  \centering
  \footnotesize
  \caption{Efficient SAM Variants: Backbone and Key Features.}
  \label{tab:efficient_sam_variants}
  \begin{tabular}{l p{3cm} p{8cm}}
    \toprule
    \textbf{Variant} & \textbf{Backbone} & \textbf{Key Features} \\
    \midrule
    %SAM 2             & Hiera (ViT)     & Streaming memory for video segmentation. \\
    FastSAM           & YOLOv8-Seg (CNN) & All-instance segmentation then prompt-guided selection. \\
    SqueezeSAM        & CNN             & U-Net based encoder-decoder architecture. \\
    EfficientSAM      & ViT-Tiny/Small  & Retrain lightweight ViT encoder with SAM leveraged. \\
    RMP-SAM           & Light CNNs      & Unified dynamic decoder with multi-task adapters. \\
    MobileSAM         & TinyViT (ViT)   & Encoder-only distillation from SAM. \\
    Light HQ-SAM      & TinyViT (ViT)   & Merge MobileSAM’s efficiency with HQ-SAM’s quality. \\
    ESAM              & EffiFormerV2 (ViT) & Holistic distillation from an expert model. \\
    NanoSAM           & ResNet (CNN)    & Knowledge distillation and TensorRT acceleration. \\
    RepViT-SAM        & RepViT (CNN)    & ViT-inspired CNN design and efficient distillation. \\
    EdgeSAM           & RepViT (CNN)    & Prompt-in-loop distillation and embedding of priors. \\
    EfficientViT-SAM  & EffiViT (ViT)   & Apply linear ReLU attention to cut computation. \\
    FastSAM3D         & ViT-Tiny   & Extends SAM to 3D with sparse flash attention. \\
    SAM-Lightening    & ViT-Tiny   & Dynamic layer-wise distillation for faster inference. \\
    RWKV-SAM          & MBConv + VRWKV  & Integrate linear RWKV operation for efficiency. \\
    TinySAM           & TinyViT (ViT)   & Hierarchical sampling with full-stage distillation. \\
    PTQ4SAM           & ViT             & Post-training quantization with adaptive granularity. \\
    PQ-SAM            & ViT             & Group activations for efficient quantization. \\
    SlimSAM           & ViT             & Structured pruning using disturbed Taylor importance. \\
    SuperSAM          & ViT             & One-shot NAS combined with pruning. \\
    SAMfast           & ViT             & Native PyTorch optimizations yield an 8× speedup. \\
    Lite-SAM          & Lite-ViT (Hybrid) & Multi-scale pooling and AutoPPN for prompt generation. \\
    MobileSAMv2       & ViT              & Object-aware prompt sampling. \\
    AoP-SAM           & ViT              & Adaptive prompt prediction with coarse-to-fine sampling. \\
    \bottomrule
  \end{tabular}
\end{table*}
